To be or not to be? an exploration of continuously controllable prompt engineering

As the use of large language models becomes more widespread, techniques like parameter-efficient fine-tuning and other methods for controlled generation are gaining traction for customizing models and managing their outputs. However, the challenge of precisely controlling how prompts influence these models is an area ripe for further investigation. In response, we introduce ControlPE (Continuously Controllable Prompt Engineering). ControlPE enables finer adjustments to prompt effects, complementing existing prompt engineering, and effectively controls continuous targets. This approach harnesses the power of LoRA (Low-Rank Adaptation) to create an effect akin to prompt weighting, enabling fine-tuned adjustments to the impact of prompts. Our methodology involves generating specialized datasets for prompt distillation, incorporating these prompts into the LoRA model, and carefully adjusting LoRA merging weight to regulate the influence of prompts. This provides a dynamic and adaptable tool for prompt control. Through our experiments, we have validated the practicality and efficacy of ControlPE. It proves to be a promising solution for control a variety of prompts, ranging from generating short responses prompts, refusal prompts to chain-of-thought prompts.

==> chap/1_intro_bak.tex <==
\section{Introduction}
\label{sec:intro}

In natural language processing, the role of prompts in guiding model behavior is well-established. A carefully crafted prompt can significantly shape the responses generated by language models\cite{liu2023gpt}. However, a one-size-fits-all approach to prompts may not always yield the desired results. For instance, a prompt designed to elicit short and concise answers can lead to overly terse responses, potentially sacrificing vital information. Conversely, In the context of retrieval-based question and answering, there are instances where the model may not accurately answer questions based on the retrieved context. In such cases, it becomes necessary for the model to learn how to effectively decline to answer questions it cannot address. However, the introduction of a refusal-to-answer prompt may inadvertently lead to the rejection of questions that the model is actually capable of answering.

\mukai{what have previous works done to solve these problems？ Need a new paragraph. Some related work should be cited here.}

To address this challenge, we introduce a method that leverages LoRA\cite{hu2021lora} to weight prompts effectively. LoRA, or Low-Rank Adaptation of Large Language Models, is a training methodology designed to expedite the training of large language models while minimizing memory consumption. It achieves this by introducing rank-decomposition weight matrices, known as update matrices, to the existing model parameters, and subsequently, only training these newly added weights.\mukai{No need to deep into LoRA itself} LoRA has shown promise in influencing the response style of models. Our key insight is to use LoRA to control the impact of prompts on model behavior, allowing for precise adjustments in response to various prompts.

We present a three-step methodology: first, we generate targeted prompt distillation\cite{sahu2023promptmix,anil2020large} datasets, then train LoRA models on these datasets in purpose of distilling the prompt into the LoRA parameters, and finally, we tune LoRA's merging weight\cite{yang2023adamerging,zhang2023composing} to achieve prompt weighting. Our experiments reveal the utility of this approach in optimizing model responses, be it for providing short and concise answers or handling refusal prompts. This research offers a flexible and powerful tool for tailoring model behavior, paving the way for more nuanced and context-aware responses in natural language processing.
\mukai{Contributions need to be organized and listed}
